Jet physics in ALICE

This work aims at the performance of the ALICE detector for the measurement of high-energy jets at mid-pseudo-rapidity in ultra-relativistic nucleus--nucleus collisions at LHC and their potential for the characterization of the partonic matter created in these collisions. In our approach, jets at high energy with E_{T}>50 GeV are reconstructed with a cone jet finder, as typically done for jet measurements in hadronic collisions. Within the ALICE framework we study its capabilities of measuring high-energy jets and quantify obtainable rates and the quality of reconstruction, both, in proton--proton and in lead--lead collisions at LHC conditions. In particular, we address whether modification of the jet fragmentation in the charged-particle sector can be detected within the high particle-multiplicity environment of the central lead--lead collisions. We comparatively treat these topics in view of an EMCAL proposed to complete the central ALICE tracking detectors. The main activities concerning the thesis are the following: a) Determination of the potential for exclusive jet measurements in ALICE. b) Determination of jet rates that can be acquired with the ALICE setup. c) Development of a parton-energy loss model. d) Simulation and study of the energy-loss effect on jet properties.

==> srcs/chapter_gersum.tex <==
% $Id: chapter_gersum.tex,v 1.2 2005/07/01 20:45:35 loizides Exp $
%

%---------------------------------------------------------------
\chapter*{Zusammenfassung}
\thispagestyle{empty}
\pagenumbering{roman}
%---------------------------------------------------------------
Diese Arbeit bestimmt die experimentellen Möglichkeiten von \acs{ALICE}, 
Jets mit einer transversalen Energie von mehr als $50~\gev$ in 
Bleikernkollisionen bei einer Schwerpunktsenergie von $\snn=5.5~\tev$ pro 
Nuk\-leonpaar zu messen. %\acs{ALICE} ist eines der vier vorgesehenen 
%Detektorsysteme am derzeit in der Bauphase befindlichen \ac{LHC}.

Für die Jetrekonstruktion werden insbesondere die Spurfindungsdetektoren, bestehend aus 
\ac{ITS}, \ac{TPC} und \ac{TRD}, benötigt. Sie befinden sich in dem  zentralen
 Akzeptanzbereich, $-0.9 \leq \eta \leq 0.9$, innerhalb eines Magnetfeldes von $0.5$~T. 
Zudem gibt es den Vorschlag, diesen zentralen Bereich durch ein \ac{EMCAL} mit einer 
Akzeptanz von $\abs{\phi}\le120^\circ$ und $\abs{\eta}\le0.7$ zu erweitern.

Wir vergleichen daher die Rekonstruktionsmöglichkeiten unter Beteiligung verschiedener 
Detektorsysteme in zentralen \PbPb\ und in reinen \pp\ Kollisionen für Jets mit 
$\Etj\gsim 50~\gev$, deren Achse innerhalb $\abs{\eta}\le0.5$ liegt.

Die Jetidentifikation erfolgt in beiden Fällen mit dem gleichen Algorithmus (\acs{ILCA}). 
Jedoch entstehen in zentralen \PbPb\ Ereignissen starke Korrelationen, die vorwiegend durch die 
zahlreiche Produktion von Minijets bei kleinen Energien ($\Etj\lsim10~\gev$) verursacht werden.
Ihre Anwesenheit macht es notwendig, den typischen Jetfragmentationsradius in der Ebene aufgespannt 
von Pseudorapidität ($\eta$) und Azimuthalwinkel ($\phi$), $R^2=\eta^2+\phi^2$,
von $R=0.7$ auf $R=0.3$ zu verringern. Zusätzlich erfordert die \mbox{hohe} Teilchendichte in 
zentralen Kollisionen, %(in der Simulation mit \acs{HIJING} sind  es um die $6000$ geladene Teilchen 
%pro Rapiditätseinheit vorwiegend bei kleinen Transversalimpulsen), 
geladene Teilchen mit $\pt<2~\gev$ nicht bei der Jetrekonstruktion zu berücksichtigen.

Mit diesen Einschränkungen sind Jets mit $50~\gev$ und höher auch in zentralen \PbPb\ Kollisionen 
identifizierbar. Doch ist ihre Energieauflösung begrenzt durch intrinsische Fluktuationen in der 
Jetfragmentierung, Teilchenproduktion außerhalb des limitierten Jetkegels, sowie Fluktuationen 
im verbleibenden Minijetuntergrund. 
%Das gilt auch für einen idealen Detektor und für Jets mit  weitaus höherer Energie. 
Ohne \ac{EMCAL} %ist die Auflösung vorwiegend dominiert durch Fluktuationen 
%im Verhältnis von geladenen Teilchen zu neutralen Teilchen in der Jetfragmentation. 
werden im Durchschnitt $50$\% der Energie rekonstruiert, mit einer Breite von $50$\%. 
Mit dem \ac{EMCAL} erhöht sich das Verhältnis zu $60$\% bei einer Breite von $30$\%.
In beiden Fällen ist die räumliche Auflösung der Jetachse (in $\eta$ und $\phi$) besser 
als $0.01$. %Die räumliche Auflösung steigt moderat mit höherer Jetenergie, wohingegen
%die Energieauflösung dominiert durch intrinsische Fluktuationen relativ unabhängig von 
%der Jetenergie ist. 
Der durchschnittliche Beitrag des Untergrundes innerhalb des reduzierten Kegels ist beträchtlich 
($15$\% bei $50~\gev$).

Bei Jets mit weniger als $50~\gev$ wird es zunehmend schwieriger, daß Signal vom Untergrund
zu trennen. In diesem Energiebereich, in dem Jetraten relativ hoch sind, werden inklusive
Meßmethoden zur Anwendung kommen. In \PbPb\ Kollisionen fällt die Rate produzierter Jets 
innerhalb der zentralen Akzeptanz von einem Jet pro Ereignis mit \mbox{$\Etj\ge20~\gev$}
auf ungefähr einen Jet in 1000 Ereignissen mit \mbox{$\Etj\ge100~\gev$}. Auf Jets mit mehr 
als $50~\gev$ sollte man daher mittels des \acp{HLT} triggern.

\enlargethispage{1cm}
Unsere Analyse zur Meßbarkeit von Jet Quenching im Rahmen eines einfachen Models
zeigt im Vergleich zu der Referenzmessung in \pp, daß die Jeteigenschaften deutlich durch den 
Untergrund der zentralen Schwerionenkollision beeinflußt werden, sogar bis zu Energien von 
$100~\gev$. Allerdings verschwindet der Einfluß mit steigendem Energieschwellenwert für die 
rekonstruierten Jets in der Analyse, und die meisten Observablen zeigen zumindest 
moderate Abhängigkeit von den gewählten Mediumsdichten.

